MULDEF: Multi-model-based Defense Against Adversarial Examples for Neural Networks

Despite being popularly used in many applications, neural network models have been found to be vulnerable to adversarial examples, i.e., carefully crafted examples aiming to mislead machine learning models. Adversarial examples can pose potential risks on safety and security critical applications. However, existing defense approaches are still vulnerable to attacks, especially in a white-box attack scenario. To address this issue, we propose a new defense approach, named MulDef, based on robustness diversity. Our approach consists of (1) a general defense framework based on multiple models and (2) a technique for generating these multiple models to achieve high defense capability. In particular, given a target model, our framework includes multiple models (constructed from the target model) to form a model family. The model family is designed to achieve robustness diversity (i.e., an adversarial example successfully attacking one model cannot succeed in attacking other models in the family). At runtime, a model is randomly selected from the family to be applied on each input example. Our general framework can inspire rich future research to construct a desirable model family achieving higher robustness diversity. Our evaluation results show that MulDef (with only up to 5 models in the family) can substantially improve the target model's accuracy on adversarial examples by 22-74% in a white-box attack scenario, while maintaining similar accuracy on legitimate examples.

==> generalframework.tex <==
\section{Our General Framework}
%In this section, we first define some terminologies used to explain adversarial examples and how to evaluate attack and defense approaches.
%\subsection{Terminology}
%
%For a certain image classification task $t$, we define the following terms:
%
%\noindent \textbf{Sample space} $\mathbb{S}$: the set of all images in the sample space.
%
%\noindent \textbf{Label space} $\mathbb{L}$: the set of all labels/classes in the classification task $t$. For example, we have 10 labels, each of which represents each digit (0-9) for a digit classification task. Thus, $\mathbb{L} = \{0, 1, 2, \dots, 9\}$.
%
%\noindent \textbf{A classifier} $f$ for the classification task $t$ can be defined as a function that takes as input an image in $\mathbb{S}$ and outputs the class in $\mathbb{C}$ for the image.
%
%\noindent \textbf{Legitimate examples} $\mathbb{N}$: the set of all normal image examples that occur naturally~\cite{Meng2017MagNet} for the classification task $t$. Thus, $\mathbb{N} \subseteq \mathbb{S}$. During the training process of neural network models, we assume that the training set and test set contain only legitimate examples.
%
%The class for each example for the task $t$ is determined by human judgment. Normally, the dataset being used to train a classifier for the task contains each example along with its class in $\mathbb{L}$ (derived with human judgment).
%
%\noindent \textbf{An adversarial example} $x$ for the classification task $t$ and the classifier $f$ is the example that is not legitimate ($x \notin \mathbb{N}$) and the classifier $f$ mispredicts the class of $x$.
%

